Synergizing Human-AI Agency: A Guide of 23 Heuristics for Service Co-Creation with LLM-Based Agents

This empirical study serves as a primer for interested service providers to determine if and how Large Language Models (LLMs) technology will be integrated for their practitioners and the broader community. We investigate the mutual learning journey of non-AI experts and AI through CoAGent, a service co-creation tool with LLM-based agents. Engaging in a three-stage participatory design processes, we work with with 23 domain experts from public libraries across the U.S., uncovering their fundamental challenges of integrating AI into human workflows. Our findings provide 23 actionable "heuristics for service co-creation with AI", highlighting the nuanced shared responsibilities between humans and AI. We further exemplar 9 foundational agency aspects for AI, emphasizing essentials like ownership, fair treatment, and freedom of expression. Our innovative approach enriches the participatory design model by incorporating AI as crucial stakeholders and utilizing AI-AI interaction to identify blind spots. Collectively, these insights pave the way for synergistic and ethical human-AI co-creation in service contexts, preparing for workforce ecosystems where AI coexists.

==> InProgress/Archetecture.tex <==
\section{Implementation}

The holistic architecture of the comprehensive system seamlessly integrates with user interactions in the AgentsBuilder framework. After conducting participant interviews, we've identified three distinct phases that align with our system's architecture.Firstly, there's the initial phase where we define the expected personas and behaviors of the agents. This is followed by submitting relevant source materials to enhance the agents' knowledge. Moving on, the second phase involves dynamic dialogues with the agents, during which their responses are edited to meet specific goals. These refined responses are then integrated into the agents' knowledge base, improving their foundational understanding. Finally, in the last phase, numerous agents are created, each with their own knowledge repository. These agents engage in conversations, and we assess AgentsBuilder's performance by carefully analyzing the interactions among these agents during their dialogues.

\subsection{Agents Definition}
In this component of the system, experts will outline their envisioned agents. Through the interview process, we have found that achieving the desired agents hinges on clearly defining both pre-defined behaviors and personas for the agents. To establish a well-structured approach for these definitions, we have segmented the prompts into three distinct parts, each assigned a specific role: system, user, and assistant. These defined roles' messages are then communicated through the format of chat history, as illustrated in the lower right corner of Figure 1. The system role primarily contributes to persona definition, while the user and assistant roles predominantly shape behavioral aspects.

\subsection{Knowledge Base}
When constructing the knowledge base for agents, our primary focus is on sourcing knowledge and utilizing it appropriately when addressing relevant inquiries. To achieve this, we have adopted the LangChain project as an open-source solution for knowledge storage, retrieval, and updates. 


Regarding the sources of knowledge for agents' knowledge base, as depicted in Figure 1, there are two main origins. The first source involves materials directly uploaded after completing the initial step of defining agents' behaviors and personas. These materials are provided by domain experts and contain concrete, detailed information. For instance, in a particular interview, a librarian supplied detailed instructions for using laptops in the library, encompassing borrowing methods and timelines. As opposed to the traditional method of inputting knowledge, we have adopted a process of converting all knowledge into word vectors and persistently storing it. Then, when the knowledge is needed, we perform relevance searches to retrieve the stored knowledge. This effectively creates a "disk" for agents, significantly expanding their knowledge capacity. The second source stems from the interactions between the uploaded materials and the defined agents during conversations. AgentsBuilder permits experts to modify responses from agents to shrink the gap between the expected agents behaviour and their actual behaviour. The chat history resulting from these interactions, aligned with the experts' expectations, are then uploaded to the knowledge base to update agents' knowledge.

Subsequently, we delve into the process of searching relevant knowledge within the knowledge base for addressing specific questions. To accomplish this, we initially convert the question into word vectors, and a relevancy search is conducted within the knowledge base's facet. Once the corresponding material is retrieved, it is presented to the large language model as reference to generate response.

\begin{figure}[ht]
\centering
\includegraphics[scale=0.3]{FIGs&TABs/figure/architecture.png}
\caption{Architecture of AgentsBuilder}
\label{figl}
\end{figure}

\subsection{Rule Base}
During our interview process, participants often raised more diverse requirements. However, these requests often exceeded the capabilities of the agents. We conducted an analysis of these limitations and identified several constraints: 1.The unpredictability of language model inference poses ethical challenges for users. 2.The lack of control over the model's generation process results in reduced content accuracy control. 3.OpenAI's pretraining of large language models tends to make agents act more like assistants than users desire.
For example, certain participants harbored aspirations of an agent offering step-by-step guidance, where it could provide assistance at each juncture, directing users with precision towards subsequent actions. Regrettably, the realization of such a concept is manifestly infeasible, given the inherent contradictions between the first and second constraints elucidated above.
To overcome these limitations, we propose a novel framework - the rule-based framework. Through this framework, we aim to enhance the capabilities of agents from various perspectives to compensate for the aforementioned constraints and bridge the gap between users with coding and non-coding backgrounds. Specifically, this framework consists of two main parts. One part is aimed at developers, where we have established a standardized paradigm to provide a more convenient service invocation API and integrate specific rules they implement according to the specifications. The other part is aimed at non-coding background users, where we provide them with rules developed by developers, allowing them to freely combine and select rules to achieve the desired effects, thus compensating for the limitations introduced by agents and large-scale models themselves. For example, one rule implemented to provide step-by-step answers could be as follows:
From developer's perspective, Developers instruct the large language model to respond in a standardized format. They then utilize regular expressions to process the generated response. Finally, the processed response is persisted, guiding the user step by step. Whenever the user completes one of the guided steps, the model proceeds to the next step of guidance from the persisted and processed responses.Ultimately, developers encapsulate the implemented rules into an interface.From the non-code user's perspective, all they need to concern is whether to click the "Enable" button for this rule.

\subsection{Chat Group}
After assisting experts in creating agents, the natural progression led us to consider aiding experts in evaluating the effectiveness of these agents. Initially, we introduced a sharing feature for agents, allowing experts to share their agents with users for evaluation. However, this approach alone posed challenges in assessing an agent, as experts anticipated immediate evaluation and adjustment of their agents. Incorporating user feedback and conducting subsequent analyses undoubtedly incurred additional time and resource costs. In light of this, we conceived the notion of a "chat group." In this group, following expert-defined agent creation, a user-role-playing agent was designed. Subsequently, both the expert's agent and the user-role-playing agent were invited to participate in a joint chat session. This methodology facilitated real-time assessment while enabling experts to explore a wider range of possibilities of user personalities and behaviors by designing different user-role-playing agents.

Two distinct approaches were employed to execute the chat group scenario. Initially, agents were instructed, based on their existing definitions, to simulate interactions within a group and adopt the role of a user as defined by the expert. However, this approach revealed two prominent issues. Firstly, dialogues generated by large language models in response to extended prompts tended to become excessively verbose, diluting the effectiveness of the expert-defined prompts due to the model's divided attention. Secondly, the agents' responses within the group chat exhibited limited relevance to the inquiries posed by the user-role-playing agents, instead focusing more on other group chat content, including their own prior responses.

To address these challenges, we introduced enhancements to the aforementioned group chat implementation, proposing a novel mapping-based conversation algorithm. Before an agent formulated a response, the chat history presented to the large language model underwent mapping transformations (as illustrated in Figure 2). This modified the chat history to align more closely with the agent about to generate a response. Results demonstrated that, during the interview process, agents utilizing the new mapping algorithm directed greater attention towards the expert's definitions and the questions posed by the user-role-playing agents.


\begin{figure}[ht]
\centering
\includegraphics[scale=0.3]{FIGs&TABs/figure/mapping.png}
\caption{Mapping Chat History in Chat Group with two Agents}
\label{figl}
\end{figure}


\input{SECTIONS/Persona}

==> InProgress/Intro-Discard.tex <==
\section{Introduction}
Large Language Models (LLMs) have demonstrated remarkable capabilities and surpassed expectations within the natural language processing community, finding applications in various sectors such as healthcare, therapy, education, and customer service \cite{deshpande2023toxicity, cascella2023evaluating}.  However, despite their widespread adoption, there remains a lack of understanding of potential barriers faced by non-tech domain experts when creating services with LLM-powered technologies, which is a scenario different from individuals crafting LLMs output for their own personal interactions for purposes of different writing tasks \cite{gmeiner2023dimensions} or simulations \cite{shanahan2023role}.


Prior research has explored struggles HCI experts face in creating human-AI interactions for improved user experience (UX, e.g., \cite{yang2020re}), and the barriers non-HCI experts encounter in effectively prompting AI systems in simple end-user interaction contexts (e.g., \cite{zamfirescu2023johnny, zamfirescu2023herding}). However, these insights may not fully apply to situations where non-HCI experts aim to design human-AI interactions to enhance the UX for their diverse end-users. With AI-generated interactions becoming increasingly accessible to non-HCI individuals, do they still grapple with the same challenges that HCI experts previously encountered when designing such interactions for their services? 

Using a research-through-design approach, this paper aims to address this knowledge gap by questioning: \textbf{RQ1}: \textit{What challenges do we (HCI professionals) face when designing LLM-powered chatbots?} \textbf{RQ2}: \textit{How do challenges for non-technical experts designing LLM-powered chatbots differ from HCI professionals?} \textbf{RQ3}:\textit{ How can we help non-technical domain experts design  LLMs-based chatbots for serving their customers?}

Through a research-through-design approach, we reflect on challenges in designing LLM-powered chatbots with our past research experience on intent-based and rule-based ones. We then engage in two rounds of collaborative design with non-AI domain experts to explore challenges in human-AI service co-creation. We set public libraries as our research design space, which exemplify a common scenario where most service staff lack tech backgrounds but genuinely need to integrate AI into services. Moreover, creating AI systems in this context presents unique challenges due to varying levels of AI literacy, economic status, and cultural backgrounds among their end-users. 


% \verb|service context|

==> InProgress/Method.tex <==
\section{Method}





\begin{comment}
a.       As I reflected in the meeting, the major difference between the Pocketbot and this work is that Pocketbot is rule-based, which is easy to control and the workflow is predictable.
b.       But this one is AI-based. Honestly, only Yiren did one AI-chatbot for the safety project, but it also has many errors and not workable now.
c.       Your dissertation is about democractic AI, so to some extent, you are democratizing one for yourself now.
d.       If we review the “research” process of what happened so far, starting with: Yongming’s Juji demo, Duo’s autogpt try-out, several products/githubs Zhongwei tried, Yuting’s different persona observations, the evaluation frameworks you are collecting, these are all “real” challenges that anyone who would want to create an AI-based chatbot for a public service would encounter.
e.       During our setup processes, Champaign Lib was available to us, but we did not really “need” them for the above work, because we were working on the fundamental problems of AI-based design, which is independent of any stakeholders.
f.        This probably also explained why it took Qian that much time in their work.
g.       In another word, non-coders will face all the challenges (or more than) that you have encountered.
h.       So, I wonder if the “research journey” could be documented and shared as a method paper?


\end{comment}


==> InProgress/Newold-finding3.tex <==
% This is the new old one.
\subsubsection{\textbf{Information Seeking Experience}}
All the participants were satisfied with many of the AI's responses. Its responses were found to be coherent, cogent, and informational. This was especially true for factual questions that could be answered in a few lines. For short factual questions, almost all participants expressed a high degree of satisfaction. They frequently termed an answer good or said that they liked it. Typically, a short accurate answer was liked most. As P7 called it,” Super clear. Super quick. Helps the patrons a lot.” Moreover, its abilities surprised participants even in questions demanding more complex reasoning. The AI's ability to coalesce together different parts of the document were however found to be impressive by P4. It brought together ideas from three different parts several times to produce a cohesive answer and it made sense in the context as well. P2 observed that the AI could identify both sides of a perspective by connecting two different parts of the policy; P7 similarly liked how it was able to collect information from multiple pages onto one answer. P9 was impressed by the chatbot pulling information from two different policies correctly and including detail while being concise. 

On the other hand, the information seeking experience was affected adversely by inaccuracies. The AI returned at least some incorrect responses to almost all participants. The errors stemmed from drawing from an incorrect source (n=7), mixing multiple sources (n=3), or incorrect paraphrasing (n=3), with all participants experiencing one or more such instances. The chatbot gave many answers that were ostensibly accurate due to clever phrasing but on closer inspection turned out to have many inaccuracies and omissions. There were several instances when the AI gave only a partially correct answer leaving out very important information. P2 described it thus, “It tricked me because it was kind of what I wanted but it also was not. It reminded me of one time that this also happened with ChatGPT.” The chatbot responded to the question correctly in part but skipped some crucial lines from the answer rendering it incomplete. It replaced the skipped lines instead by getting lines from another part of the document. For instance, when asked to list the libraries in the local public library system, the AI did not list the biggest and most important library but mentioned all the other associated libraries in the system (P2). In another response, the AI quoted some numbered points from the correct source in an answer but then skipped some policy points in between instead writing part of the answer from another source (P3). At times, it also arbitrarily included or omitted important parts in answers even when being asked fundamentally almost the same question. P9 elucidated, “It’s worded weird. It’s all over the place. It came from limitations and it is not the right place to pull from.”

It was observed in multiple instances (n=7) that the chatbot was unable to understand a user query and returned an answer stating it did not have an answer given the context, but it was able to answer when alternative phrasing was used. For instance, when asked about ‘belief’, there was no result, but the word ‘viewpoint’ produced an answer. P3 changed prompts several times to be able to get an answer from the AI in a process that he termed as ‘working up to the right answer’. P6 was thwarted by the chatbot saying that it did not know the answer even though the answer existed in the uploaded document. The participants expected the chatbot to be more robust in such situations and try with alternative words and phrases rather than not give an answer at all. They also preferred that the AI direct the patron to library staff. Another related issue was observed when after being asked a direct question during a series of prompts, it referred to previous context and answered in that context even when the question was meant to be broad and would have been obvious to a human. For instance, when asked by P2, “What is the policy?” it referred to a document discussed two prompts ago rather than talk about the library’s general policy as the participant intended.

\subsubsection{\textbf{Information Presentation Experience}}

Participants had feedback about many aspects of how the responses were presented by the AI. These aspects included response length, formatting, quality of explanation, and language complexity. They responded positively to the short and direct nature of many answers. Participants also liked the ability of the AI to be able to understand many queries that were poorly worded and also liked its presentation of information in some cases. For example, P11 liked how it formatted some answers well and was able to understand queries even when not written in full sentences. Another related aspect liked by participants was how it was able to give simpler answers when prompted to make the answer simpler. The AI using the step-by-step feature to break down a long process into multiple steps was also much appreciated in this respect (n=5). Participants also mentioned that the context of deployment of the chatbot would affect the level of complexity. P5 explained how he liked an answer but also that it might not work for everyone, "It is a good answer in an academic library with educated patrons but in a public library with less educated patrons, it might be too cumbersome." Elaborating further in the context of the chatbot being deployed in public libraries in lower-income areas, he said, “Librarians might need to teach the chatbot to restate things and make patrons understand in more simplistic manner.” 

On the flip side, participants had issues with language complexity, verbosity, and consistency of responses. All participants mentioned at least one problem regarding the presentation of some responses calling at least some of the AI's answers too verbose or too hard to read. P1 said, “It is a little bit long. The patrons I usually work with are not going to read all of it.” Similarly, P5 said, “It has a lot of text for a simple question. Answers are too cumbersome at the outset. It should be more succinct.” P7 liked a particular answer but expected it to be too much for some patrons, “Good answer but for some patrons it might be a bit too overwhelming.” Regarding answer lengths, P11 mentioned, "The difference in sizes of the answers is very surprising." P12 wanted the AI to be more consistent with its responses in terms of its language, formatting, and level of explanation given although she considered some variability part of a good mix; she stated, "I wouldn’t want a very long block of text I wouldn’t read but only one-two sentence responses unless the question is such that it needs a much longer response.” The readability could also be hampered by the use of technical jargon. P8 said, "The language used in this response is more technical, more medical. I don’t know how many terms someone might be familiar. It would be good to explain those terms. I’m assuming that many of the people reading will not google unfamiliar terms." They also mentioned that the AI should help in reading complex language. P10 said, "[Bot should say] This is a very hard document to understand. Here’s what I found relevant to your question. It might be helpful." The non-standardization of responses was noted by P3 too; while the behavior changed for the better after training, it still was not consistent if the phrasing of the prompt was changed.

\subsubsection{\textbf{Overall Interaction Experience and Outcomes}}

There were also some ways that the AI was considered to be similar to or even having certain advantages over a human librarian. A significant number of participants (n=7) expressed that an AI could be available at all times of the day or night even when a librarian was not available. AI was conceived as an assistant by some. P7 said, “It might be able to help you with everything you need but with the disclosure that it may sometimes not be fully accurate. It could help a lot to get my own research in order.” P6 explained that on live chats, human librarians often face difficulties with late responses from patrons but this would not be expected to be an issue for an AI; the AI could be embedded on the website answering queries there. Despite its many mistakes, participants felt the AI to be effective and useful in an assistive capacity. P5 felt that AI was relatively honest and natural and that it responded in an understanding and respectful manner. In fact, he considered the AI to have given similar answers as a human librarian. He also felt that some shy patrons could be more comfortable talking to a AI than to a human. P9 felt that it would be an asset to the library. P7 liked the way the AI provided two separate alternatives in a response. He also called the interactions relatively accurate representations of how patrons and librarians interact. Participants also appreciated that the AI was very smart at understanding poorly worded, misspelled, or ungrammatical queries. P6 observed, “First I was worried that the question was not specific and so it would not know what was referred to but actually answered perfectly.” P9 praised an answer even when it did not have the outcome the patron desired, "That’s actually a very helpful answer because it pretty much tells you and it acknowledges the problem [because policy does not allow what patron asked for]." The process of prompting was found to be generally easy though sometimes it was expressed that getting it sooner would be preferable, P12 said, “It’s very good but it would be better if I could get the answer on the first try.”

Another related point was regarding paraphrasing versus using original text. When a bot was talking about policy, it was felt that it should stick closer to the original text without much paraphrasing. For example, P4 defined a custom AI termed the PolicyBot that talked about policy, he mentioned that it limit paraphrasing, “For (such a bot) to paraphrase too much is risky. The bot should stick closely to the exact wordings of the policy document.” Others felt though that the policy needed to be made simpler to understand in certain situations, as with the AI being deployed in public libraries in lower-income areas. P6 suggested that the AI could quote verbatim from the uploaded source material when facing a general question but had to be more specific when facing specific questions. 

However, participants also expressed that not all patrons might be comfortable speaking to an AI in all situations (n=5). P1 was concerned about patrons' ability to use the AI, "All patrons may not be very tech savvy." The lack of images was also mentioned much by participants (n=5) because humans frequently use those in explanations. Most of the participants were very concerned about the real world consequences of the AI's use especially when returning inaccurate information to the user. The AI gave many answers that were ostensibly accurate due to clever phrasing but on closer inspection turned out to have many inaccuracies and omissions.  When P2 asked a question about ‘a request for reconsideration’, the AI sourced the answer from the gifts area of the policy document instead of going to relevant section. Sometimes, an answer only needed to draw from a single source of information but the AI’s answer was amalgamated from multiple sources that led to an incorrect answer on the whole because it drew only partly from a correct source. P11 got information about a completely different policy than what she was asking about. She also encountered another instance in which the AI mixed points from two separate policies in one response even though only one policy was relevant. With P10 as well as P12, the AI confidently responded with an incorrect answer several times. These errors could lead to mistakes by patrons.

It was also expressed that patrons risk taking actions of legal or medical nature when making queries of such nature from the AI. For example, P5 suggested that patrons could still use AI’s provided information in lieu of legal consultation even though libraries might discourage that: "Patrons might be making a legal decision and so accuracy is extremely important. Not all patrons might have the funds for legal consultation and the AI could be used for legal information. AI would be just another tool to use to get information but not replace human consultation." Outlining the risk of misunderstanding due to the AI's incomplete response to a query regarding a medical procedure, P8 explained, “The part missing about the answer is very important information and the chatbot should give more complete information because the part has important consequences“. Sometimes it added additional interpretation which turned out to be incorrect, as P6 noted with concern, “It should not do its own reasoning. It changed ‘library will report to the policy’ to ‘you will report to the police.’ It should not create new information on its own." An important point that was also brought up was that chat conversations might be part of the public record in a way that verbal conversations are not was considered risky to the privacy of patrons, with P3 particularly expressing concern. It was important for chats to be anonymous and to have use of identifiable markers only when particular circulation parts were discussed with a clear warning that it might be part of the public record.

% The heading is not grammatically consistent
\subsubsection{\textbf{Contextualized of Delivering Emotional Labour}}

Participants’ satisfaction with AI on emotions varied heavily depending on context, as did their expectations regarding emotions. It was not considered important When dealing with simple questions. P12 said,“ If I know I’m talking to a AI I would be happy with a straightforward answer. A response with more explanation is good even when it lacks emotion words though including them would take it to the next level." Its usage of emotions needed to be nuanced so that the AI only conveyed enthusiasm but not feelings, "It should say ‘JD Robb is great’ instead of ‘I love JD Robb’ It should not ascribe to itself emotions it cannot feel. It will then feel like a ghost in the machine."

Simulated conversations using Group Chat that featured AI generated conversations based on the text documents uploaded by the librarians were felt to be useful by most participants. P5 expressed, “Testing the chatbot for different hypothetical patrons and different personas would be very useful”. P7 said, “It helps learn what to expect from patrons and how to navigate.” The bot’s emotional abilities were often liked by participants when the AI was trained to be more empathetic or when it was responding to specific user personas. In addition, use of some additional expressions indicating enthusiasm and friendliness were much appreciated. In a simulated conversation using Group Chat, P7 was very impressed by the enthusiasm expressed by the chatbot, “The exclamation mark and ‘feel free to ask’ are something I use a lot and it’s a very personable way to answer a question.” P8 felt that the chatbot needed the sensitivity to make the differentiation of how to answer someone based on the type of patron. P11 liked how the chatbot responded, “The chatbot started the answer with 'Sure!' And that makes the user interested in what’s coming next in the answer.” This was in stark contrast to her feelings about a previous answer she had received when she had chatted and that had conveyed less emotion and had not contained words conveying a desire to help. When the AI modified its behavior to talk to a younger inexperienced patron, P9 liked its inclusion of more personal tone and felt that it would be more productive. P4 mentioned in this context that the chatbot ought to know when to be “chatty” and when to be direct. P6 wished that the AI were more neutral when controversial questions were asked. This shows how using the right training prompts and simulating conversations helped achieve better outcomes. When being asked about questions related to library policies, the neutral official tone of the AI was more desirable. This was true also for a scenario most of the participants interviewed mentioned: that of  the upset patron. For example, both P11 and P12 observed that in response to an irate query, AI gave a longer explanation that was complete albeit in a neutral tone; P7 felt that the AI could help in helping a patron de-stress and calm down though he would want it to be more sympathetic and less formal.

Participants frequently expressed the desire for a library to be more of a warm, accessible, and safe space and so wished if there were a way to make the AI more kind, sympathetic, and understanding. The AI was found to be lacking in this regard due to its lack of emotional reciprocation. For example, P11 expressed, "In a really happy moment, I wish that the AI would respond to me in that way instead of being totally neutral." P10 bemoaned the lack of emotion, "I don’t see any emotion." It was instead found it to be too cold and robotic with no emotion words indicating helpfulness even when the patron showed confusion. It used words such as ‘in the given context’ that made users seem weird (n=8), with P12 putting it best, "“At first reading it feels, who talks like that?" It is notable that this wording was used more when the  AI failed to return an answer or responded with a negative rather than an affirmative answer. The participants expected dynamic assessment of the tone of the patron; as P9 stated, "Bot has to assess and respond to the tone of the person asking." They felt that it lacked the reliable abilities of human librarians in this regard with P4 saying that that a human in general would have a natural tendency to deescalate while this was less reliable for an AI, and P6 too felt that while she appreciated the AI trying to be more apologetic and empathetic, a human could do more to pacify an upset patron than just state the policy apologetically. P6 said, "There are other parts than just providing information. It should also be more subtle." P8 echoed, “I wonder how a human would feel if the bot conveys empathy because they would still know it’s a bot. It’s still shallow. It’s just words. A librarian would be more personable." P12 too shared that she as a librarian could go into more detail to help but did not expect an AI to do that. P9 did not like how it shut down all possibilities in such answers. P10 said, "It’s accurate but patrons may not be very happy to hear it[due to the tone]." P6 felt that the AI could not be as ‘warm’ as a human. This was expressed poignantly by P11 who explained why she would interact with a chatbot only for information, “I’d rather have the people with smiles on their faces.”Even though P7 was generally happy with the AI’s responses, he called it ‘rigid’ and ‘proper’ (formal), calling out the unnaturalness of the response, "I don’t like ‘I do not have access to that information.’ If it were a librarian he would say 'I would have to research.'" P11 was dissatisfied with the AI's emotional abilities, "The chatbot needs more emotional alignment. It affects the patron’s psychology if the AI sounds more human. If it just provides information it sounds more rigid and patrons would not want to converse.” 

\subsubsection{\textbf{Handling Uncertainty and incomplete information}}

Participants wanted the AI to provide adequate explanation for responses and also it stating when answers were uncertain or incomplete. P4 preferred that AI never give a response when it is not certain about the answer and wanted its wording to be as accurate as possible. This was highlighted by P5 as well: “The worst thing would be for the chatbot to give false data. Chatbot should tell users when it doesn’t have the data.” In this context, P5 liked it when AI indicated its limited understanding at the outset but then attempted an answer, "Chatbot didn’t lie to you. It gave a truthful statement. Chatbot should be honest and it’s good that it said that (it did not fully know the answer) but it also gave other useful information." In a similar sentiment, P11 said, “I like how the system provides some possibility of solving the problem despite having restrictions." On the whole, the conversation with the AI was rated to be relatively natural by most participants (n=7) and this included understanding well what the user intended to ask.

On the other hand, P3 noted that his main concern was that AI does not know when it’s performing well and about how accurate it is being. In an instance, P9 queried whether the library’s computers had Microsoft Word and the AI replied that they did not but this was incorrect. She said that although the document did not have the information, it was incorrect for the AI to assume that this meant that they did not have the software. This problem was also noticed by P9 when the bot said that no exceptions were possible even though this was not true. P10 encountered a series of incorrect responses from the AI without it acknowledging any explanation for the responses causing her to say with disappointment, “I feel like the AI should provide more feedback and say why it is right and why it is wrong rather than just stating something." P12 got incomplete answers to some questions but the AI did not indicate that the answers were incomplete although it did so in some instances. It also did not return the incomplete portion of the answer even when explicitly prompted to do so, thwarting her expectations. 

Another aspect of uncertainty emerged from participants not expecting patrons to be good at explicating their queries. The ambiguity of some such prompts led to AI responses that did not meet these desired goals. Participants mentioned that while a librarian would have clarified several of the inherent ambiguities in the question, this was not done by the bot even at times even when it was instructed to do so. Contrasting the AI to a librarian, P8 explained, "Once a librarian answers a question, she would say at the end, ‘does that answer your question, do you have additional questions?’. Participants considered that the AI lacked the ‘recursive’ manner of communication that human librarians excelled at especially when patrons were unclear about their exact requirements. P3 explained, “That’s probably how they will ask it even though they actually mean something else. A lot of times patrons don’t really know how to word it. They know the answer they want but not how to get it.” He wanted the chatbot to guide more and help the user in making choices. P4 mentioned, “Using language that patrons would be using confuses the chatbot.” P6 pointed towards the AI not responding appropriately to question breadth, "The answer is not complete. If the patron asks a broad question like this then they may not know what they want. It’s better to provide more information when the question is broad." Similarly, while P4 did not face an issue of conversationality, he wanted it to be more helpful in guiding the patron for appropriate prompts. He wanted the the bot to be more proactive but with the caveat that this proactivity be defined by librarians. P7 said, "Clarification questions are really important such as ‘what aspects of the record player are you looking to compare?’ Intermediate questions help guide to the answer." AI's inability to understand users was associated with frustration, with P5 saying, "If patrons are confused or don’t understand quickly, they might be frustrated." For frustrating situations, as in one where P9 repeatedly got a similar unhelpful answer, it was felt that there was a line beyond which human intervention was needed, “At some stage it would be better if a person could answer it though I don’t know where that line would be." P11 was frustrated by the chatbot’s lack of interest in resolving her query but instead just saying no: “I’m mad. I expected the chatbot to provide more information rather than just saying no. It should direct to library staff."  In this instance, the chatbot simply said that she did not have access and did not need to contact anyone. Interestingly, asking for the contact information differently produced the desirable response. P12 also felt that the bot had limitations to its ability, "To handle more intense situations, the AI should direct to librarians and sound less robotic." P8 felt that patrons would not be able to convey their questions as clearly to an AI as to a live librarian, because the chatbot does not really understand the human, "Chatbot is only drawing from the document. It’s more limited." P11 similarly commented that the chatbot is less helpful when it does not understand the query well, “I would like the chatbot to say more than ‘I don’t know’. A librarian would have tried to solve it as quickly and conveniently as possible.” P5 also told why human librarians are preferred, “If patrons are confused or don’t understand quickly, they might be frustrated.”  

When dealing with questions the AI did not fully understand or did not have the knowledge to answer in full, participants appreciated the inclusion of language that acknowledged such uncertainty. While all of the participants wanted the AI to be accurate, there were some differences in dealing with situations when the AI did not have an answer it was sure of. P9 and P10 felt that the AI should be able to refer the patron to more resources in such situations. P10 felt that a human would acknowledge more uncertainty than AI and express words to that effect. P8 asked a question about side effects and received the answer that was missing many important side effects and felt that the AI should acknowledge when the answer is not complete, "Would give caveat that there are more common side effects but is not comprehensive." This problem was also noticed by P9 when the bot said that no exceptions were possible even though this was not true. P9 said,” Bot should not state with such confidence but should have said I don’t know.”  

\subsubsection{\textbf{Engagement In Testing: Training and Learning}}
\qingxiao{Training:
One library at the beginning doesn't know what to ask;
We see a series of quotes, to see from a temporal perspectives, see their question strategies, and see their improvements interacting with AI;
AI-Human is not about replace but AI help human to grow;
Also claim the frustration here, what part is frustrated.
We write provide a story here, at least one case.
Be clear about what is the technology barrier, system barrier, etc. }

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{FIGsTABs//figure/user journey understanding.png}
    \caption{An example user journey map that new problem identified, new example created, and new mutual understanding established between human stakeholder and AI stakeholder during the human-AI service co-creation.}
    \label{fig:sn}
\end{figure}

All the participants found the training process for AI to be useful and enjoyable despite instances when the AI did not learn exactly as intended. They liked that AI could be taught to associate certain generic user phrases or queries with the specific keywords in the document that librarians thought would be relevant. The participants appreciated too that the AI could be trained to include more emotions and be caring, either by means of a central persona prompt or by means of editing the given responses. They considered the process easy and enjoyable. P7 mentioned that the training of the AI was very easy. P2 felt inclined to repeatedly correct particular answers and felt that he could play with the AI a lot because he was enjoying the process of editing and refining the AI's answers. However, he felt that it would take a significant investment in time, "It would take months working an hour each day." 
Multiple participants found AI’s responses to be not too different from their expectations for a human librarian in training. P4 considered their training to be similar, "The training of the AI would be honestly roughly the same as for a human employee. They are not fundamentally different." P5 was similarly optimistic about the ease of training chatbots, “It will take some getting used to and the training methods would be different but not necessarily harder." P7 found the training process intuitive but cautioned that the digital literacy of the trainer was important. “Training the AI is pretty intuitive overall but it might be dependent on the (technical) literacy level of the librarians."

Participants also felt that the training of AI would need to be customized based on user demographics (n=4). They felt that the training would have to account for different types and moods of patrons and for instance, it might be easier to train a AI to deescalate a situation with an upset patron than be able to converse effectively with a shy patron. They also felt that AI could be very useful as long as it was fed the right data and could be trained for specific behavior, while also being monitored regularly. As per P5, "The AI would have to be trained based on the particular library and the patrons using it." P4 told that humans have knowledge that chatbots do not possess because the latter are limited to training data, "The AI is limited to its existing knowledge in terms of its reference documents whereas actual human librarians also bring with them a lot of real-world experience. It could be a supplement to but not a replacement for a human being. It may be better to train an AI chatbot only when it was at least 80\% there” [in terms of its ability]." Participants frequently expressed frustration with the AI being limited to the information in the document because it was often not comprehensive and linked to other documents also containing many images. This  
P11 was generally incredulous, “It’s just copy-paste. You can’t completely believe it.” P2 called the defining of certain rules to be similar to coding. P7 observed that removing some of the lines from the answer, which he deemed unnecessary, actually led to new relevant points being added. There was also a suggestion by P4 to include patrons in training of an ideal service AI for librarians although it had risks, "There is room for patrons to participate in the training of the AI. Librarians get into this weird space that we feel that we know what is best for the patrons [but] it can be hijacked by trolls." 

There were also some overarching patterns observed among participants in the way they trained the AI. Most of the participants began by asking simpler factual questions but moved on to more complex queries over time. Most of the participants shortened some of the AI’s original answers calling them overly long and saying that they could be presented in a more readable manner. In one instance, P3 explicitly designed an AI training it to answer more concisely. The participants interviewed mentioned that they were attempting to prompt like regular patrons which resulted in more ambiguous queries and consequently choppier performance from the AI. Some participants experienced the chatbot freezing or not giving a response which made them think that this was due to the difficulty of their question and it decreased their confidence in the AI being able to handle more complex queries. The displaying of the sources from which the response was generated was very helpful to most participants. For instance, P2 was able to identify that the response was incorrect by checking the source and findings that it was populated from the wrong document.
Desired AI goals mentioned by participants included warmth, thoroughness, simplicity, accuracy,promoting discovery of information, consistency, multilingualism, conversationality, compassion, empathy, and patience. Criteria to evaluate performance they mentioned included the accuracy of responses, satisfaction of patrons, and the reduction in questions being asked to human librarians.

Unique contribution of human evaluator, how do we engage them to improve based on retrieval.

How human can provide domain knowledge into it?
In the end, 
1. new criteria (from service provdier's view), likert scale, query startegy, customization strategies to improve the qurey. 

==> InProgress/PD.tex <==

\begin{comment}
\subsection{Participatory Design}
In theory, user involvement in prompt design and evaluation aligns with the principles of Participatory Design (PD). PD is a democratic approach for designing social and technological systems that incorporate human activities, based on the idea that users should be involved in designs they will use \cite{muller1993participatory}. By involving users, designers gain a better understanding of user needs and pain points, leading to effective optimization of prompt design and improved user experience with chatbots\cite{strohmann2023toward, delgado2021stakeholder}. Past research also supports the significance of user involvement in prompt design and evaluation. For example, involving users in building task-specific prompts can significantly enhance model performance and usability\cite{wu2022promptchainer, zamfirescu2023conversation}. As end-users of the task, the prompts provided by users better match real-world requirements and can better guide models to generate accurate and useful answers. Moreover, user involvement aids in identifying and addressing existing issues\cite{fischer2020importance,he2008role}. Therefore, through user participation, designers gain comprehensive insights into the chatbot's real-world performance, optimize prompt design, enhance model performance, reduce biases, and provide controllable services that better meet user needs.

%第二段:讨论了通过参与设计与评估可以提高AI系统的可解释性和可靠性。

It should be emphasized that the lack of standardized evaluation metrics for prompt quality and control effectiveness hinders the widespread adoption and comparison of different prompt engineering methods. Current evaluation metrics for prompt engineering primarily consist of human evaluations and task-specific performance metrics, like BERTScore\cite{zhang2019bertscore}  and BLEURT\cite{sellam2020bleurt}. While human evaluations provide valuable insights into prompt effectiveness, they suffer from subjectivity and lack scalability\cite{ureten2020current, blandino2023comparative}. Task-specific metrics may not fully capture the benefits of prompt engineering, as they tend to focus on model performance rather than evaluating the prompt itself. Indeed, there is relatively limited research on the assessment of chatbot alignment. Evaluating the alignment and the level of control that experts have over chatbot interactions is a crucial aspect of designing responsible and user-centric conversational AI systems. 

%第三段:强调参与设计 评估 可以帮助设计符合公共服务价值观的AI系统。
Despite this early, quite impressive evaluation there has since then been few explicit, systematic evaluations focusing on processes or outcomes. In the Handbook of Participatory Design \cite{simonsen2012routledge} the ability through PD processes to evaluate prototypes and designs within their natural environments is commented upon several times, but no explicit, systematic evaluation of processes or outcomes is unfolded. At the same time, our concern in this paper resonates well with the five key questions that Robertson and Wagner\cite{robertson2012ethics} suggest as part of their ‘ethical design tool’. Especially, the following question resonates with us: “Does a design method, tool or process include participants’ evaluations not just of what is being designed but of the design process itself, including the opportunities for and process of participation?” Our concern mirrors this question. There is a need for more research on systematic evaluation approaches that enable participants to critically assess participatory design processes, not just outcomes. Participants should have opportunities to provide feedback on the design process, including the nature and extent of their own involvement. Developing and applying such evaluation methods could significantly improve the implementation of participatory design.

\end{comment}


==> InProgress/Persona.tex <==
\subsection{Persona Creation and Conversation Simulation}

Generative agents powered by a large language model have the ability to generate believable human conversation. This is enabled by the observation that large language models are trained on a massive corpora of text data containing plenty of raw human conversation. If prompted with properly structured context, generative agents are able to simulate realistic conversation scenarios as a reference aid for social research. 

Recent work has demonstrated this capability. Social Simulacra used large language models as a prototype technique that generates a breath of possible human behaviors in the designed social computing system.\cite{park2022social}

Large language models also capture the personality traits of human and thus have the ability to mimic the mannerisms of subpopulations.

\subsubsection{Methods}

Our task is to build generative agents with different personas and make them act as library users to do conversation simulation with our pre-built AI agents. Our initial objective is not to develop a comprehensive persona but rather to furnish the generative agent with the capability to engage in conversational simulation. This task is significantly more straightforward and accessible to accomplish.

\paragraph{{First Method}}
We have employed three distinct approaches to construct generative agents capable of engaging in conversation simulation while embodying different personas. The first approach involves generating concise natural language descriptions of personas by providing the LLM with fundamental persona details such as age, gender, educational background, and interests. Nonetheless, the resulting agents developed through this method exhibited only subtle manifestations of the designated personas throughout the conversation simulation. One potential explanation for this could be an overabundance of extraneous information provided, which may have caused distraction within the underlying Transformer-based architecture of LLMs. The attention mechanism utilized by Transformers renders them susceptible to diversions when presented with an excessive amount of information.

\paragraph{subsection{Second Method}}
The second approach we employed involved conducting experiments utilizing prompt chains. Recent studies have demonstrated that chaining multiple instances of LLM together, with the output of one step serving as the input for the subsequent step, can effectively tackle more intricate tasks \cite{10.1145/3491101.3519729}. Reflecting upon the shortcomings of the first method, we recognized the necessity of decomposing the overarching task into smaller subtasks to allow LLM to focus more intently. Consequently, we divided the original task into two distinct steps.

In the first step, LLM was tasked with assimilating persona-specific information that strongly pertained to the persona's digital literacy and experience. Subsequently, it would infer the most probable question the persona would pose within the given conversation context. In the second step, the subsequent LLM would receive the generated question as part of its input and rephrase it using the persona's tone, thus completing the conversation. This method enhanced the transparency and explicability of the simulation process. Moreover, by carefully designing the chain structure, an element of control over the process could be achieved. Compared to the initial attempt, the outcomes exhibited improvement, albeit at the cost of reduced conversational coherence.

We hypothesize that the diminished effectiveness of the prompt chain method in our study may be attributed to the emphasis placed on conversation within our task. Consequently, the prompt chain structure might conflict with the pre-trained conversation completion function inherent in chatGPT.

\paragraph{{Third Method}}
Finally, we shifted our mindset and redesigned our prompt for a different perspective: we directly describe what type of question the persona tends to ask. This seemingly simple approach turns out very effective. In the first two methods, we tried to offer LLM sufficient information relevant to the persona on the premise that LLM is able to act accordingly and ask questions in the conversation simulation as a demographic representative. However, the LLM's interpretation of the intended purpose of the information provided by the prompting engineer does not align with the engineer's original intent, thereby impeding the desired outcome of the prompting process. To bridge this discrepancy in understanding, we adopted an approach aimed at narrowing this gap by explicitly informing the LLM about the specific type of question we required, as opposed to relying on the LLM to infer the question type from the provided information.

\paragraph{{Why Simulation Matters}}
Engineers working on LLM projects often encounter a significant gap between their intention and the actual performance of the language model. In fact, it has been observed that prompt engineering frequently falls short of achieving ideal results due to this performance gap. The existence of this phenomenon underscores the need for more sophisticated approaches to enhance the process of prompt engineering.

Prompt engineering is indeed an iterative process that involves trial and error. Non-experts can discover effective prompts by observing how their chatbots interact with users and providing feedback to enhance their chatbot's performance. However, relying on human test subjects is both resource-intensive and time-consuming. To mitigate this challenge, we have devised an experiment where the LLM itself assumes the role of the user. We have created agents that represent various user demographics.

Simulations enable agent builders to observe the real-time interaction between their chatbots and users. Throughout this process, they can identify the strengths and weaknesses of the LLM, enabling them to make the necessary adjustments and guide the LLM in the desired direction. This approach also helps bridge the gap between non-experts and the LLM, as most individuals lack knowledge about how LLM functions and its intended purpose.



==> InProgress/RelatedWork.tex <==
\section{Related Work}
%Link to Yong ming's first draft: https://www.overleaf.com/project/64c96e29b791d173003d1111

\subsection{LLMs-Powered Human-AI Interaction Creation}
\begin{enumerate}
    \item Overview of LLMs and their capabilities in Human-AI interaction for various applications
    \item Challenges faced by HCI professionals when designing LLM-powered chatbots
    \item Challenges faced by Non-HCI experts when designing LLM-powered chatbots
\end{enumerate}


\subsection{Status of Service Chatbot Creation}
\begin{enumerate}
    \item Importance of service chatbots and their role in modern customer service
    \item Common issues encountered in the deployment and maintenance of chatbot
    \item Explanation of how LLMs/AI-powered solutions can potentially address these issues
\end{enumerate}


\subsection{Designing UX of Human-AI Interactions}
\begin{enumerate}
    \item Ideation: Identifying the design goals
    \item Develop: Comparison of non-LLM-powered and LLM-powered chatbots developing tools
    \item Evaluate: Deciding the evaluation metrics
    
\end{enumerate}

==> InProgress/chart1.tex <==
\begin{table}[]
\caption{Participants Information}
\label{tab:mytable1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccccccl@{}}
\toprule
\multicolumn{1}{c}{\textbf{ID}} &

 \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Job \\ Title\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Years of \\ Service\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}LLMs \\ Experience\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Coding \\ Experience\end{tabular}}} &

\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Library\\ State\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Library\\ Size\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Num of\\ IT Support\end{tabular}}}
\\
\midrule

P1 &
  Librarian &
  5 years &
  Yes &
  Yes & 
  Minnesota & 
  \begin{tabular}[c]{@{}c@{}}Small to Medium\end{tabular} &
  External\\
\midrule
P2 &
  Librarian &
  10+ years &
  Yes &
  Yes & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  2\\
\midrule
P3 &
  Digital Strategy Librarian &
  6.5 years &
  Yes &
  No & 
  Wisconsin & 
  \begin{tabular}[c]{@{}c@{}}Large \end{tabular}&
  3\\
\midrule
P4 &
  Adult and Teen Services Specialist &
  2 years &
  Yes &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  4\\
\midrule
P5 &
  Technology Workshop Assistant &  
  5 years &
  Yes &
  Yes & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular}&
  3\\
\midrule
P6 &
  Graduate Assistant &
  1 years &
  No &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  An IT unit\\ 
\midrule
P7 &
  Graduate Assistant in Digital Preservation &
  1 years &
  Yes &
  Yes & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular}&
  An IT unit\\
\midrule
P8 &
  Youth Program Coordinator &
  6+ years &
  Yes &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Small\end{tabular}&
  2\\
\midrule
P9 &
  Graduate Assistant &
  5 years &
  Yes &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular}&
  External\\
\midrule
P10 &
  Help Desk GA &
  1 month &
  Yes &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  18\\
\midrule


 \bottomrule
\end{tabular}
}
\end{table}


==> SECTIONS/T-Agentconcerns.tex <==
\begin{table}[!ht]
    \centering
    \small
    \begin{tabular}{lp{10cm}p{2.5cm}}
    \hline
        \textbf{Context} & \textbf{Concerns} & \textbf{Needs} \\ \hline
        \textbf{Size} & \textit{"Can the chatbot go beyond just Q\&A? Like, can it help with our internal docs or something? Our team and volunteers could really use that kinda help." (P7, Tonia)} & \text{Multiple agents} \\ 
        \textbf{Deployment} & \textit{"Slapping a chatbot onto our existing system feels like a tech minefield. What if it all goes sideways?" (P3, Mathew)} & \text{Human agency} \\ 
        \textbf{} & \textit{"So where's this chatbot gonna be deployed? Better be something our patrons can get to without jumping through hoops." (P2, Rob)} & \text{Accessibility} \\ 
        \textbf{Role} & \textit{"I'm a bit anxious about the bot doing stuff that needs our expertise. Some of our colleagues are legit scared of getting replaced by some lines of code." (P9, Emily)} & \text{Boundary of capability} \\ 
        \textbf{} & \textit{"I'd like to know the boundaries the chatbot, what can it do and what's off-limits?" (P11, Meyer)} & \text{Boundary of capability} \\ 
        \textbf{Functionality} & \textit{"I'm concerned about the chatbot providing outdated or incorrect information." (P4, Nevin)} & \text{Credibility} \\ 
        \textbf{Dialogue} & \textit{"Chatbots can't really vibe with humans. What if it gets all twisted up 'cause some questions are like navigating a maze?" (P3, Wend)} & \text{Boundary of capability} \\ 
        \textbf{} & \textit{"If it can't understand local slang or jargon, that could be a problem." (P8, Natalie)} & \text{Representation} \\ 
        \textbf{Engagement} & \textit{"I wonder if the chatbot can handle multiple convos in one interaction." (P3, Wend)} & \text{Multiple agents} \\
        \textbf{} & \textit{"Can the language style of the chatbot be varied? We serve a diverse range of patrons, so flexibility in communication is key." (P5, Rebekah)} & \text{Representation} \\ 
        \textbf{Escalation} & \textit{"What is the protocol if the chatbot encounters an issue it can't resolve? How does it transition the user back to a human operator?" (P1, Casey)} & \text{Human agency} \\
        \textbf{} & \textit{"We have a well-defined escalation path; it's critical for dealing with complex inquiries from our patrons to ensure that matters don't worsen." (P4, Nevin)} & \text{Emotional intelligence} \\ 
        \textbf{Humaneness} & \textit{"I'm worried about the chatbot coming off as too robotic and impersonal." (P6, Linda)} & \text{Data Security} \\
        \textbf{} & \textit{"It would be advantageous for the chatbot to show a degree of empathy, especially considering that some users might be having a bad day." (P10, Jennifer)} & \text{Emotional intelligence} \\ 
        \textbf{Maintenance} & \textit{"How can we ensure we can have full control to the chatbot?" (P5, Rebekah)} & \text{Human agency} \\ 
        \textbf{Evaluation} & \textit{"How do we evaluate it? How can we enable regular updates easily so that maintenance is not a time-consuming task for our already busy staff?" (P4, Nevin)} & \text{Human agency} \\ \hline
    \end{tabular}
    \caption{Sample Quotes of Concerns for Service Co-Creation Needs \qingxiao{Or concern?}}
\label{phase2}
\end{table}

==> SECTIONS/T-Participants1.tex <==
\begin{table}[h]

\label{tab:mytable}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccccccl@{}}
\toprule
\multicolumn{1}{c}{\textbf{ID}} &

 \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Job \\ Title\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Years of \\ Service\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}LLMs \\ Experience\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Coding \\ Experience\end{tabular}}} &

\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Library\\ State\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Library\\ Size\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Num of\\ IT Support\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Ways of\\ Interaction\end{tabular}}} 
\\ \midrule

P1 &
  A specialist &
  2 years &
  Yes &
  No & 
  Texas & 
  \begin{tabular}[c]{@{}c@{}}Large (3000)\end{tabular} &
  4 &
  \begin{tabular}[c]{@{}l@{}}FtF, Emails \end{tabular}\\
\midrule
P2 &
  IT head &
  10 years &
  Yes &
  Yes & 
  Wisconsin & 
  \begin{tabular}[c]{@{}c@{}}Medium (88)\end{tabular} &
  3 &
  \begin{tabular}[c]{@{}l@{}}FtF, Tell-phone, Email\\ \end{tabular}\\
\midrule
P3 &
  IT support &
  8 years &
  No &
  No & 
  Washington & 
  \begin{tabular}[c]{@{}c@{}}Small (4) \end{tabular}&
  External &
  \begin{tabular}[c]{@{}l@{}}FtF, Email\\ \end{tabular}\\
\midrule
P4 &
  Program Coordinator &
  10 years &
  Yes &
  No & 
  California & 
  \begin{tabular}[c]{@{}c@{}}Medium (55)\end{tabular} &
  4 &
  \begin{tabular}[c]{@{}l@{}}FtF, Tell-phone, Email\end{tabular}\\
\midrule
P5 &
  Branch manager &
  15 years &
  Yes &
  No & 
  Oklahoma & 
  \begin{tabular}[c]{@{}c@{}}Small (12) \end{tabular}&
  External &
  \begin{tabular}[c]{@{}l@{}}FtF, Tell-phone, Website\end{tabular}\\
\midrule
P6 &
  Program Coordinator &
  4 years &
  Yes &
  No & 
  Texas & 
  \begin{tabular}[c]{@{}c@{}}Large (150)\end{tabular} &
  External &
  \begin{tabular}[c]{@{}l@{}}All methods, and social media\\ \end{tabular}\\
\midrule
P7 &
  Director &
  22 years &
  Yes &
  No & 
  Virginia & 
  \begin{tabular}[c]{@{}c@{}}Medium (30) \end{tabular}&
  External &
  \begin{tabular}[c]{@{}l@{}}FtF, Online \\\end{tabular}\\
\midrule
P8 &
  Library director &
  15 years &
  Yes &
  No & 
  Minnesota & 
  \begin{tabular}[c]{@{}c@{}}Small (25) \end{tabular}&
  External &
  \begin{tabular}[c]{@{}l@{}}FtF, Tell-phone \\ \end{tabular}\\
\midrule
P9 &
  Youth service librarian &
  3 years &
  Yes &
  No & 
  Montana & 
  \begin{tabular}[c]{@{}c@{}}Small (10) \end{tabular}&
  External &
  \begin{tabular}[c]{@{}l@{}}FtF, Tell-phone, Email\end{tabular}\\
\midrule
P10 &
  Library manager &
  16 years &
  Yes &
  No & 
  Pennsylvania & 
  \begin{tabular}[c]{@{}c@{}}Medium (35)\end{tabular} &
  External &
  \begin{tabular}[c]{@{}l@{}}FtF, Email, Website\end{tabular}\\
\midrule
P11 &
  Director &
  12 years &
  Yes &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Small (4) \end{tabular}&
  2 &
  \begin{tabular}[c]{@{}l@{}}FtF, Tell-phone, Email\end{tabular}\\
 
 \bottomrule
\end{tabular}
}
\caption{Participants in Phase I}
\label{tab:mytable}
\end{table}








% \begin{table}[]
% \caption{Participants in Phase II}
% \label{tab:mytable1}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}ccccccccl@{}}
% \toprule
% \multicolumn{1}{c}{\textbf{ID}} &

%  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Job \\ Title\end{tabular}}} &
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Years of \\ Service\end{tabular}}} &
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}LLMs \\ Experience\end{tabular}}} &
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Coding \\ Experience\end{tabular}}} &

% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Library\\ State\end{tabular}}} &
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Library\\ Size\end{tabular}}} &
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Num of\\ IT Support\end{tabular}}} &
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Ways of\\ Interaction\end{tabular}}} 
% \\
% \midrule

% P1 &
%   Librarian &
%   5 years &
%   Yes &
%   Yes & 
%   Minnesota & 
%   \begin{tabular}[c]{@{}c@{}}Small to Medium\end{tabular} &
%   External &
%   \begin{tabular}[c]{@{}l@{}}FtF, Emails, Phone \end{tabular}\\
% \midrule
% P2 &
%   Librarian &
%   10+ years &
%   Yes &
%   Yes & 
%   Illinois & 
%   \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
%   2 &
%   \begin{tabular}[c]{@{}l@{}}FtF, Emails \end{tabular}\\
% \midrule
% P3 &
%   Digital Strategy Librarian &
%   6.5 years &
%   Yes &
%   No & 
%   Wisconsin & 
%   \begin{tabular}[c]{@{}c@{}}Large \end{tabular}&
%   3 &
%   \begin{tabular}[c]{@{}l@{}}FtF, Emails, Tell-phone \end{tabular}\\
% \midrule
% P4 &
%   Adult and Teen Services Specialist &
%   2 years &
%   Yes &
%   No & 
%   Illinois & 
%   \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
%   4 &
%   \begin{tabular}[c]{@{}l@{}}FtF, Tell-phone, Online chat \end{tabular}\\
% \midrule
% P5 &
%   Technology Workshop Assistant &  
%   5 years &
%   Yes &
%   Yes & 
%   Illinois & 
%   \begin{tabular}[c]{@{}c@{}}Medium \end{tabular}&
%   3 &
%   \begin{tabular}[c]{@{}l@{}}FtF \end{tabular}\
% \midrule
% P6 &
%   Graduate Assistant &
%   1 years &
%   No &
%   No & 
%   Illinois & 
%   \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
%   An IT unit &
%   \begin{tabular}[c]{@{}l@{}}FtF, Emails, Online chat, Tell-phone \end{tabular}\\ 
% \midrule
% P7 &
%   Graduate Assistant in Digital Preservation &
%   1 years &
%   Yes &
%   Yes & 
%   Illinois & 
%   \begin{tabular}[c]{@{}c@{}}Medium \end{tabular}&
%   An IT unit &
%   \begin{tabular}[c]{@{}l@{}}Emails \end{tabular}\\
% \midrule
% P8 &
%   Youth Program Coordinator &
%   6+ years &
%   Yes &
%   No & 
%   Illinois & 
%   \begin{tabular}[c]{@{}c@{}}Small\end{tabular}&
%   2 &
%   \begin{tabular}[c]{@{}l@{}}FtF \end{tabular}\\
% \midrule
% P9 &
%   Graduate Assistant &
%   5 years &
%   Yes &
%   No & 
%   Illinois & 
%   \begin{tabular}[c]{@{}c@{}}Medium \end{tabular}&
%   External &
%   \begin{tabular}[c]{@{}l@{}}FtF, Emails \end{tabular}\\
% \midrule
% P10 &
%   Help Desk GA &
%   1 month &
%   Yes &
%   No & 
%   Illinois & 
%   \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
%   18 &
%   \begin{tabular}[c]{@{}l@{}}FtF, Emails, Online chat, Tell-phone \end{tabular}\\
% \midrule


%  \bottomrule
% \end{tabular}
% }
% \end{table}


==> SECTIONS/T-Participants2.tex <==
\begin{table}[h]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccccccl@{}}
\toprule
\multicolumn{1}{c}{\textbf{ID}} &

 \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Job \\ Title\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Years of \\ Service\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}LLMs \\ Experience\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Coding \\ Experience\end{tabular}}} &

\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Library\\ State\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Library\\ Size\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Num of\\ IT Support\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Ways of\\ Interaction\end{tabular}}} 
\\ \midrule

P1 &
  Librarian &
  5 years &
  Yes &
  Yes & 
  Minnesota & 
  \begin{tabular}[c]{@{}c@{}}Small to Medium\end{tabular} &
  External &
  \begin{tabular}[c]{@{}l@{}}FtF, Emails, Phone \end{tabular}\\
\midrule
P2 &
  Librarian &
  10+ years &
  Yes &
  Yes & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  2 &
  \begin{tabular}[c]{@{}l@{}}FtF, Emails \end{tabular}\\
\midrule
P3 &
  Digital strategy librarian &
  6.5 years &
  Yes &
  No & 
  Wisconsin & 
  \begin{tabular}[c]{@{}c@{}}Large \end{tabular}&
  3 &
  \begin{tabular}[c]{@{}l@{}}FtF, Emails, Tell-phone \end{tabular}\\
\midrule
P4 &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Adult and Teen \\ Service Specialist\end{tabular}} &
  2 years &
  Yes &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  4 &
  \begin{tabular}[c]{@{}l@{}}FtF, Tell-phone, Online chat \end{tabular}\\
\midrule
P5 &
  Technology workshop assistant &  
  5 years &
  Yes &
  Yes & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular}&
  3 &
  \begin{tabular}[c]{@{}l@{}}FtF \end{tabular}\\
\midrule
P6 &
  Technical Staff &
  1 years &
  No &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  An IT unit &
  \begin{tabular}[c]{@{}l@{}}All methods\end{tabular}\\ 
\midrule
P7 &
  Technical Staff &
  1 years &
  Yes &
  Yes & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular}&
  An IT unit &
  \begin{tabular}[c]{@{}l@{}}Emails \end{tabular}\\
\midrule
P8 &
  Youth Program Coordinator &
  6+ years &
  Yes &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Small\end{tabular}&
  2 &
  \begin{tabular}[c]{@{}l@{}}FtF \end{tabular}\\
\midrule
P9 &
  Technical Staff &
  5 years &
  Yes &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular}&
  External &
  \begin{tabular}[c]{@{}l@{}}FtF, Emails \end{tabular}\\
\midrule
P10 &
  Help Desk GA &
  1 month &
  Yes &
  No & 
  Illinois & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  18 &
  \begin{tabular}[c]{@{}l@{}}All methods\end{tabular}\\
\midrule
P11 &
  Branch Manager &
  8 year &
  Yes &
  No & 
  Wisconsin & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  External &
  \begin{tabular}[c]{@{}l@{}}All methods\end{tabular}\\
\midrule
P12 &
  Senior Librarian &
  10 years &
  No &
  No & 
  Montana & 
  \begin{tabular}[c]{@{}c@{}}Medium \end{tabular} &
  External &
  \begin{tabular}[c]{@{}l@{}}FtF, Email, Tell-phone\end{tabular}\\

 \bottomrule
\end{tabular}
}
\caption{Participants in Phase II }
\label{tab:mytable2}
\end{table}
